Identity-free Artificial Emotional Intelligence via Micro-Gesture Understanding

In this work, we focus on a special group of human body language -- the micro-gesture (MG), which differs from the range of ordinary illustrative gestures in that they are not intentional behaviors performed to convey information to others, but rather unintentional behaviors driven by inner feelings. This characteristic introduces two novel challenges regarding micro-gestures that are worth rethinking. The first is whether strategies designed for other action recognition are entirely applicable to micro-gestures. The second is whether micro-gestures, as supplementary data, can provide additional insights for emotional understanding. In recognizing micro-gestures, we explored various augmentation strategies that take into account the subtle spatial and brief temporal characteristics of micro-gestures, often accompanied by repetitiveness, to determine more suitable augmentation methods. Considering the significance of temporal domain information for micro-gestures, we introduce a simple and efficient plug-and-play spatiotemporal balancing fusion method. We not only studied our method on the considered micro-gesture dataset but also conducted experiments on mainstream action datasets. The results show that our approach performs well in micro-gesture recognition and on other datasets, achieving state-of-the-art performance compared to previous micro-gesture recognition methods. For emotional understanding based on micro-gestures, we construct complex emotional reasoning scenarios. Our evaluation, conducted with large language models, shows that micro-gestures play a significant and positive role in enhancing comprehensive emotional understanding. The scenarios we developed can be extended to other micro-gesture-based tasks such as deception detection and interviews. We confirm that our new insights contribute to advancing research in micro-gesture and emotional artificial intelligence.

==> src/declarations.tex <==
\section{Declarations}
The authors have no competing interests to declare that are relevant to the content of this article. The code and datasets generated during and/or analyzed during the current study are available at: \href{https://github.com/Erich-G/MG_based_Emotion_Understanding}{https://github.com/Erich-G/MG\_based\_Emotion\_Understanding}. 

The contributions of each author are as follows. Rong Gao: Conceptualization, Methodology, Software, Writing - Original Draft. Xin Liu: Conceptualization, Methodology, Writing - Original Draft \& Review \& Editing, Funding acquisition. BoHao Xing: Methodology, Software. Zitong Yu: Methodology, Writing - Review \& Editing. Bjorn W. Schuller: Writing - Review \& Editing. Heikki Kälviäinen: Supervision, Writing - Review \& Editing, Funding acquisition.
